Revamp: Enhancing Accessible Information Seeking Experience of Online Shopping for Blind or Low Vision Users

Online shopping has become a valuable modern convenience, but blind or low vision (BLV) users still face significant challenges using it, because of: 1) inadequate image descriptions and 2) the inability to filter large amounts of information using screen readers. To address those challenges, we propose Revamp, a system that leverages customer reviews for interactive information retrieval. Revamp is a browser integration that supports review-based question-answering interactions on a reconstructed product page. From our interview, we identified four main aspects (color, logo, shape, and size) that are vital for BLV users to understand the visual appearance of a product. Based on the findings, we formulated syntactic rules to extract review snippets, which were used to generate image descriptions and responses to users' queries. Evaluations with eight BLV users showed that Revamp 1) provided useful descriptive information for understanding product appearance and 2) helped the participants locate key information efficiently.

==> 3_investigation_1.tex <==
\section{Formative Study}
To understand the current practice and special needs of BLV users when shopping online, we conducted 30-minute semi-structured online interviews with 20 BLV consumers (native language: 10 English and 10 Chinese; gender: 7 female and 13 male; average age: 28) recruited through social media platforms. Each study was audio recorded, transcribed and coded by a group of three researchers following the reflexive thematic analysis methods from Braun and Clarke [\xx]. We summarize the results based on the questionnaires, transcripts, notes and observations.  Although the platforms and languages they use differ, participants share similar screen reader experience and information seeking challenges since the screen readers follow the general design and most online shopping websites are similarly structured with overloaded information.
The demographic information of participants is attached in the Appendix.

Specifically, the goal of this study is to understand when shopping online:
\begin{itemize}
  \item What challenges do BLV users face in information seeking and their coping approaches?
  \item What are the design heuristics for an accessible information retrieval system for BLV users?
\end{itemize}

% \xac{marked as unread}

\subsection{Challenges}
Aligned with prior work [\xx], two main challenges mentioned by our participants are lack of visual information and lack of efficient ways to navigate through information. We discussed further insights on how the challenges were related with BLV users' specific needs on understanding product appearance under the context of online shopping.
\xac{maybe mention how our study goes beyond this prior work so readers know what to look for as they keep reading}

\subsubsection{Lack of Visual Information}
The most frequently mentioned challenge is the lack of detailed information for understanding the visual appearance of the product (18 out of 20 participants). While sighted users can tell the visual attributes such as color, shape and size or even functionalities of a product from a single image, 
%BLV users depend on the alt-text of the image to understand its content. However, 
the alt-texts of many current product images are either empty, or set as the image path, which does not provide any visual information for BLV users at all.
Sellers usually provide no textual information equivalent to that conveyed by images.
Take the color attribute as an example, the names provided by sellers are usually too generic to interpret accurately and can even be very obscure sometimes. 
% \xac{up to this point, the writing seems to come from the authors' experience as there is no mentioning of participants}
P5 mentioned his story that once he wanted to buy a guitar and was curious about what exactly was the color attribute `gold'. \code{Is it a shining one or a matte one? I couldn't figure it out by myself unless there had (been) more descriptions.}
P18 brought up another example that a T-shirt with the color name \code{surf the web} was actually a kind of bright blue.

%to understand the appearances without adequate descriptions compensating for information conveyed by images.
% all about tables or other things move to discussion and results
% 4 Participants also mentioned reading comparison tables and size charts line by line can be confusing, which calls for new interaction model to access tables and charts. (out of scope, not online-shopping specific)
% Consistent with what have been revealed in prior study \cite{Stangl:2018:BOC:3234695.3236337}, our participants mentioned inaccessible web elements, \eg navigation, flowing window, etc., due to inadequate development of web accessibility guidelines.
%\code{reading tables can be confusing with a screen reader...it's just one of those things we all get used to} (P12) \code{It could be high level analysis questions based on these comparison table.} (P17)
% Alt-text for images in eCommerce sites are often empty, or simply set the same as the product name, which is not informative enough. Visual attributes in an image, such as color (Arctic blue), pattern (marble texture), style (Nordic, Instagram), when described only by text becomes far less expressive. 
%Participants also mentioned there were many cases where the sellers provided obscure attribute names. P8 brought up an example that a T-shirt with the color name \code{surf the web} was actually a kind of bright blue.
%While such naming approaches might be attractive to sighted consumers, they add extra barriers for BLV users to understand the product.
% besides color, for different categories, they care about different details, we further explore the detials in the xx section.

% move to discussion later for main categories
%This is the same case with other basic visual attributes, \eg shape, size, logo and graphics design on the product.
%Without vivid image descriptions, participants tend to avoid buying certain categories of products online, \eg clothes, home \& kitchen ornaments.
%For products such as electronics, food and toys, the information provided by the seller were usually enough for making a shopping decision. 


% to add other visual attributes
% should I move the collecting questions into this part?

%Other attributes, such as price, ingredients or functionalities, usually do not require detailed description to understand, unless the consumers are not familiar with the specialized prior knowledge about a product and need to learn from others' opinions. 


\subsubsection{Lack of efficient ways to navigate through information}
Comparing with the scanning and skimming experience of sighted users, the passive and sequential reading manner of screen readers makes it inefficient for BLV users to retrieve useful information scattering all over a web page.
P16 mentioned that it can be frustrating when accidentally jumping into another unrelated web component such as the shopping cart in the process of exploring product details. 
%which is overloaded with reviews, product information and details provided by sellers, etc. 
%\code{I know there exists a lot of useful information on the product page, but it is too clunky to find them in the clutter.} (P14)
All participants agreed that reviews were useful resources, as the snippets with detailed descriptions can provide further insights for product appearance.
%However, sifting through the large amount and often duplicated reviews can be especially laborious. 
%hence the detailed descriptions and subjective feedback from other buyers are under-utilized, including those that can provide further insights for product appearance.
%\eg “\textit{the light-colored marble pattern feels cool to use in summer}” and “\textit{this elegant marble pattern suits the white wall}” (P3).
However, most participants (16 out of 20) reported their utilization of reviews was greatly reduced because sifting through the large amount and unrelated reviews can be especially laborious. P19 mentioned that ``\textit{Usually there are too few reviews per page and there are no easy ways to jump from review to review.}''. 

%"\textit{There are too much information. Some reviews are very vague. It is quite random if I could get useful information from the reviews or not by manually navigating them one by one.}" (P4)
% \xac{this quote is more about the quality/usefulness of reviews rather than navigating reviews} (\xx). 
 
% \xac{mention this in design recom}

%\subsection{Current Approach}

%\subsubsection{Seeking Help from Sighted People}
%To overcome the challenges, most participants (80\%) choose to seek help from sighted people including families/friends, other customers and paid video chats. Amazon also provides an accessibility hotline for help.
%They would ask a product question and let the helper read related information and provide detailed image descriptions. In this way,
%they had to trust the helper's personal judgment: 
% , some participants are used to this 
%``\textit{I rarely buy clothes or other appearance-related items by myself —- I wear whatever my family bought me.}'' (P8) 
%``\textit{I'm completely trusting another person's judgment when it comes to items whose appearance matters in a subjective way.}'' (P12) A number of participants mentioned the desire to explore products by themselves, as they found their friends ``\textit{don't describe well}'' (P7) or family members interfere with their buying decisions, \eg ``\textit{stopped me from buying a pair of shoes she hated}'' (P16). Some participants (P3, P19, P20) ask the same question to different friends and compare their opinions to generate an objective impression.

%Although participants heavily rely on human help, they realized the inconvenience of this approach and hope there was an alternative solution for them to shop more independently. The most frequently mentioned concerns were unavailability, time consumption and privacy: "\textit{If I'm looking for a product description, it often takes longer for someone to get back to me than if I didn't need help.}" (P16) "\textit{Rather than receiving the product in a few days, it entirely depends on availability of the family member or friend as to when I can order the product.}" (P19) 
% "\textit{It can be inconvenient to have to wait for somebody else to be available to help me. Also, I don’t always want friends and family knowing about certain products that I buy, so I wind up not asking them even though it would be helpful.}" (\xx) 
% \xac{one quote would be enough; this is not ground-breaking finding}
%Besides, one participant mentioned he did not trust a helper without relevant purchasing experiences because ``\textit{The things I buy online, for example, electronics, often require some kind of specialized foreknowledge. If a person doesn't have that knowledge, it can happen that they give wrong, or incomplete information. This can lead to frustration and dissatisfaction.}''

% \xac{is there any new (shopping-specific) insight here? seems to be a common problem any other assistive technology is trying solve}
% \vio{seems not except the last one, but I think it can be very frustrating that the time waiting for help is even longer than receiving the product}

% \xac{highlight what findings and quotes are unique to shopping}

\subsection{Current Solutions}
\subsubsection{Seeking Help from Sighted People}
80\% participants choose to seek help from sighted people including families/friends, other customers, paid video chat and accessibility hotlines.
In this way, they had to trust the helper's personal judgment and subject to issues such as helpers' inavaliability and privacy concerns.
P19 mentioned that \code{Delivering process is not the most time-consuming for me. Waiting for someone to get back to me is.} \xac{what did P19 mean by 'delivering'?}
P12 stated that he did not always want others to know about certain products he buys and hoped there was an alternative solution to shop more independently.

\subsubsection{Leveraging Existing Web Functions and Automatic Tools}
P18 mentioned using visual interpretation apps such as Seeing AI to get brief generic descriptions on product images based on object and color detection, \eg \code{probably a close up of a red chair}.
Two participants who were more tech-savvy in web interfaces (P11, P20) mentioned using keyword-based search and filters, but these tools are under-utilized by other participants and can only remove irrelevant information on a general basis.
P8 and P13 mentioned the customer questions \& answers section supported by websites can also help with some generic details, yet it seldom covers appearance-related information, which is assumed available to sighted consumers via product images.
%  can capture a product's visual appearance directly from images.


%The customer questions \& answers section supported by websites hardly cover appearance-related discussions since sighted consumers can capture a product's visual appearance directly from images;
% Searching by keywords and using filters could help remove unrelated information, but cannot pick out the reviews containing detailed descriptions which can provide further insights to appearance.

\subsection{Design Heuristics}
\xac{suggest: Implications for Design. a heuristic would be "Product page should make it easy for BLV people to navigate information"; an implication could be a heuristic and/or a solution to realize a heuristic; what's described below sounds more like solutions}

Based on the interview results, we derived 3 design heuristics to improve the accessibility of online shopping experience. Specifically, our recommendations focus on leveraging the existing data resources on the product page, and reorganize them in a structured information flow. 

\subsubsection{Simplifying and reconstructing the webpage}
When the users’ current task is understanding a product, especially the appearance, the overloaded information and web components can become burdens for seeking visual-related description. To address this problem, we can provide an alternate view of the original page with less related information and components removed, such as shopping cart.
\xac{maybe mention that it is important to make it easy for users to switch back to the original page.}

\subsubsection{Mining information from the customer reviews to supplement a lack of visual description}
\xac{might need to iterate more ...}
%All of our participants agreed that the customer reviews was a helpful resource for understanding the product, yet they also found it was extremely tedious to use. It is thus important to extract the information and present it in a way that is easy for BLV users to navigate.
%leveraging other sources on the webpage to fill in the information asymmetry; Leverage Existing Reviews: 
Participants' responses suggest that the subjective information in reviews can be helpful for BLV people to understand the visual attributes. Just as P2 stated: "\textit{It is impossible for me to build a visual concept as you sighted people do, but I can feel what you feel. Reviews talking about the feelings when seeing the appearance are helpful for me to understand this pattern.}"
%Besides, subjective reviews provide information complementary to product description, sometimes helping to avoid misleading the consumer. 
%P4 was once confused by a description named `Arctic blue', thinking it was a light color, only to find out it was more of a dark purple.
%He mentioned if he had seen the one review that pointed out such color discrepancy, he would not have been misled by the inaccurate description.

% P\xx shared with us a story when he was confused about the color of one coat, "\textit{The attribute said it was a kind of Arctic blue. In my imagination, the Arctic blue should be some kind of light color since there are a lot of ice in arctic.}" Then he sent the product link and his question about the color to one family member, and got the reply that "\textit{it looks more like a dark purple, not blue.}" He still felt confused and spent some time on reviews until he found one consumer mentioned there has a difference between the image and the entity, and the clothes was actually dark blue. Hence, not only in understanding the appearance, as a collective wisdom, reviews can also provide opinions from consumers with purchase experiences. 

\subsubsection{Bridging passive reading and active queries to enhance web search}
\xac{i feel this heuristic seems bland and sounds similar to what Amazon already has---how is our qa different}
%Instead of passively browsing the information on the product page, 
Participants expressed preference to actively asking questions and getting answers of the product, which was usually what they did when conducting with a live person.
%Participants mentioned that responding to their specific questions is more natural way of gathering information required for making a shopping decision.
%``\textit{I can understand how the search bar works but not everyone is good at asking good questions or selecting suitable keywords to search.}'' (P17) 
%Specific questions on appearance should be supported. %``\textit{The other consumers don't ask a lot about what I am concerned, for example, the appearance. To get satisfactory answers, I have to post a new question mentioning that I am blind and please describe the details for me. Also, I am not sure how long I will wait until someone answers.}'' (P8) 
%``\textit{Some reviews are understandably visual in nature and don’t answer my questions about what exactly the product looks like to my liking.}'' (P13) 
Meanwhile, any additional assistance mechanisms should be compatible with users' current screen reader experience to support users access the original information as well. P6 commented \code{I do not completely trust in answers selected by machines in case it may not cover very well}.
%Only providing reviews snippets may not be informative enough, ``\textit{The context of reviews can be very helpful, and I often get unexpected details about other aspects of the details.}'' (P1)
%\cite{10.1145/3308561.3353773}

%There may be something only human-powered approaches can solve (gap between the performance), but when these are not available, we hope there can still be some alternative 24/7 available helpers to help with information seeking, instead of letting our BLV users wait but can do nothing. This motivates the idea of Askit.


%Human helper will also look into reviews "\textit{But I hope I could get some statistical analysis from the reviews,for example, If I am interested in the quality of one furniture,I wanna know how much positive and negative reviews area bout the quality.}" (P9)

%This supports the feasibility of leveraging the reviews, this collective wisdom as one information source. and motivates the text summarization of reviews snippets.

%Actually human helper will take time looking into reviews to find some related information since he or she haven't bought this product before.

%When exploring the product page, participants first listen to the contents of the title, as well as the basic attributes of the product provided by the seller, e.g., price, color, material, function, etc. They access these information independently using screen readers and generate an initial impression of one product. The main challenges our participants faced in this process could be divided into two aspects: First, the sequential speech-based representation is not suitable for comprehensive and dynamic product page, which makes BLV people could not "scan" the screen at a glance as sighted people do. when the user have a clear goal about the information he needs, he cannot jump directly to the targeted infos; When the user just want to browse freely, he still need to cost time on useless information.  

%Cognitive Load of Interacting with Comparison Tables

%Some product pages include tables comparing with the similar products.

%compare several products to make the final decision

%能够融合 和利用各种 信息 image reviews

%one focus here should be selecting proper related contents from reviews to answer image questions
%购物图片的描述 和 普通的场景image caption不同

%We noticed that the human helper not only pay attention tothe keyword mentioned in the user’s question, but also had adivergent thinking to include more related reviews. Besides,the human helper could have multiple rounds of dialog with theuser. The user may be elicited by the answer, then proposed aquestion related to the previous but more detailed. We considerbuilding a dynamic lexicon and support granularity extractionon subset review data to meet this goal.

%This goal was summarized based on observation on how human helper provide the fragments from reviews. We noticed that the human helper could remember what have been provided to the user and will automatically skip the similar opinions. One shortcoming is that the human could only browse from the beginning of the reviews to the end, so he could only provided related reviews in this ordering. However, among all the reviews, there may have high-related ones which should be provided as early as possible. Beside, the context could be useful. For example, when the user ask about the quality of one quilt, what is actually useful is not the simple fragment of "The quality is good" or " The quality is as expectation"(which the user would only want to know the statistical summarization), but the specific opinions on why the customer think the quality is good. The related information existed in the context of the target fragment. We consider build a scoring algorithm and provide the top related reviews, and adopt the scheme of extending the length of extracted segment. As mentioned above, what users what to hear is not repeatedly"good" or not fragments, but they do want to hear about statis-tical information, which the human helper is harder to meetthe needs.

%this builds guidelines for labeling the suitable review data for one question, based on this labeled data set we 

%Also, discuss if there have differences between different nationalities. And we will first focus on deploying our solution towards united statues Amazon BLV users. (due to existing abundant resource)

%What questions will BLV consumers ask if they can directly interact with the information? (will there be differences comparing with sighted consumers?)

% \begin{figure*}[t]
%  \centering
%   \vspace{-0.6cm}
% %  \setlength{\belowcaptionskip}{-4cm}
%  \includegraphics[width=2.0\columnwidth]{questions.png}
%  \caption{specific questions example}~\label{}
% \end{figure*}






